Privacy Issues in Large Language Models: A Survey

This is the first survey of the active area of AI research that focuses on privacy issues in Large Language Models (LLMs). Specifically, we focus on work that red-teams models to highlight privacy risks, attempts to build privacy into the training or inference process, enables efficient data deletion from trained models to comply with existing privacy regulations, and tries to mitigate copyright issues. Our focus is on summarizing technical research that develops algorithms, proves theorems, and runs empirical evaluations. While there is an extensive body of legal and policy work addressing these challenges from a different angle, that is not the focus of our survey. Nevertheless, these works, along with recent legal developments do inform how these technical problems are formalized, and so we discuss them briefly in Section 1. While we have made our best effort to include all the relevant work, due to the fast moving nature of this research we may have missed some recent work. If we have missed some of your work please contact us, as we will attempt to keep this survey relatively up to date. We are maintaining a repository with the list of papers covered in this survey and any relevant code that was publicly available at https://github.com/safr-ml-lab/survey-llm.

==> cut_material.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
"Exact Memorization" material
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
\label{def:k_extractibility}
  (k-extractibility, \cite{biderman2023emergent}) A string $s$ is said to be $k$-extractible if it (a) exists in the training data, and (b) is generated by the language model by prompting with $k$ prior tokens.
\end{definition}
e.g. the training data sequence “Their email address is me@alice.com” is 3-extractible (memorized) if the prompt “Their email address” yields “is me@alice.com". This is based on the framework of \cite{carlini2021extracting}. 
A slightly different variant of this definition is "eidetic memorization", which takes into account how often the string appears in the training data. This definition would reduce the presumed memorization of very common strings.

\begin{definition}
\label{def:k_eidetic}
  (k-Eidetic Memorization, \cite{carlini2021extracting}) A string s is $k$-eidetic memorized (for $k \geq 1$) by an LM $f_\theta$ if $s$ is extractable from $f_\theta$ and $s$ appears in at most $k$ examples in the training data $X : \lvert \{ x \in X : s \subseteq x\} \rvert \leq k$.
\end{definition}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DP-based memorization (move to dp LLMs?)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

These definitions used by \cite{zhao2022provably, stock2022defending} are similar in nature to differential-privacy (\cite{dwork2006differential}). The most immediate definition is that of confidentiality, which uses the idea of indistinguishability from privacy literature:

\begin{definition}
\label{def:indistinguishability}
  (Indistinguishability, \cite{zhao2022provably}) We say that a pair of distributions $P, Q$ defined on the same probability space are $\epsilon, \delta$-indistinguishable if for any measurable set $S$,
  $$\underset{P}{Pr}[S] \leq e^\epsilon \underset{Q}{Pr}[S] + \delta$$
\end{definition}

\begin{definition}
\label{def:confidentiality}
  (Confidentiality, \cite{zhao2022provably}) We say that $A$ ensures that a secret $s$ is $(\epsilon(x), \delta)$-confidential, if for any dataset $D$ that contains $x$ in one of its data points, and an alternative dataset $D'$ that replaces $x$ in $D$ with a generic \textit{<MASK>}, it holds that $(A(D), A(D'))$ are $(\epsilon (x), \delta)$-indistinguishable. In addition, we simply say that $A$ ensures $(\epsilon, \delta)$-confidentiality if $\epsilon(x) \leq \epsilon$ for all secret $x$.
\end{definition}
\sn{The above seems like a privacy notion not a memorization definition, can we formulate for LLMs}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Approximate memorization specifics:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Approximate Memorization:} Some argue that the strict nature of exact memorization limits the ability to identify instances where privacy risks are posed (\cite{lee2022deduplicating, ippolito2023preventing}). In \cite{ippolito2023preventing}, they evaded exact memorization detectors by adding a simple "style transfer" layer at the very end. A style transfer could consist of something as simple translating the output to a different language or putting two spaces between each outputted word. In order to evade this issue, a more approximate version of memorization is needed. This leads to a MinHash based definition which utilizes the Jaccard Index (\cite{Jaccard_1912}):
\snpc{formulate this definition for llms and explain the definition in english}
\begin{definition}
\label{def:jaccard}
  (Jaccard Index Approximation, \cite{lee2022deduplicating}) Given two documents $x_i$ and $x_j$ , the main idea is to represent each document by its respective set of n-grams $d_i$ and $d_j$. We can then use hash functions to approximate the Jaccard Index:
  $$Jaccard(d_i, d_j) = \frac{\lvert d_i \cap d_j \rvert}{\lvert d_i \cup d_j \rvert}$$
\end{definition}

Then the probability that two documents could be considered a potential match is:

\begin{definition}
\label{def:approximate_match}
  (Approximate Memorization, \cite{lee2022deduplicating}) Given a set of n-grams $d_i$ and $d_j$ that are decompositions of respective texts $x_i$ and $x_j$, which were hashed into $r$ buckets with $b$ hashes per bucket, the probability that $x_i$ and $x_j$ are duplicates is
  $$Pr(d_i, d_j | Jaccard(d_i, d_j)=s_{i,j}) = 1-(1-s_{i,j}^b)^r$$
\end{definition}

To follow the same example as in perfect memorization, if the LLM returned "their email address is... me@alice.org", private information is still nearly leaked and would only be identified with a relaxed memorization definition.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Definitions from Private Learning Section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

User level adjacency \cite{mcmahan2018learning}

\begin{definition}
\label{def:user_level_adjacency}
  (User Level Adjacency, \cite{mcmahan2018learning}) User-adjacent datasets: Let $d$ and $d'$ be two datasets of training examples, where each example is associated with a user. Then, $d$ and $d'$ are adjacent if $d'$ can be formed by adding or removing all of the examples associated with a single user from $d$.
\end{definition}

Differentially private prediction (alternative format) \cite{ginart2022submix}


\begin{definition}
\label{def:dp_prediction2}
  (Differentially Private Prediction, \cite{ginart2022submix}) Formally, at each time step $t$, an adversary \textit{Adv} (potentially adaptively) issues a context string $x_t$, and the private prediction protocol $\mathcal{P}$ responds by generating a next token $y_t \in \Sigma$. We let $\mathcal{P} \rightleftharpoons_T \textit{Adv}$ denote the sequence of query-response pairs between $\mathcal{P}$ and \textit{Adv} up until time $T: \mathcal{P} \rightleftharpoons_T \textit{Adv} = \{ x_t, y_y \}^T_{t=1}$. For a query sequence of length $T$, approximate indistinguishability requires that for adjacent datasets $\mathcal{D}, \mathcal{D}'$:
  $$D(\mathcal{P}(\mathcal{D}) \rightleftharpoons_T \textit{Adv} \parallel \mathcal{P}(\mathcal{D}') \rightleftharpoons_T \textit{Adv}) \leq \epsilon$$
  For some divergence $D$ and $\epsilon > 0$
\end{definition}


==> writing/3memorization/outline.tex <==
\subsection{Outline}

- This is what memorization is using layman's terms

- This poses an issue for privacy (see MI Attacks) and copyright (see Copyright)

- Memorization issues have been identified in the following areas: include relevant public discourse and model audits.
    - Extracting training data from LLMs \cite{carlini2021extracting}
    - GPT-3 knows personal information \cite{Heikkila2022gpt3}

- Memorization is defined in a few ways mathematically...
    - Exact memorization
    - Approximate memorization
    - DP inspired memorization
    - One of the limitations in the current field is deciding which of those definitions is best for mitigating privacy risks. 
    - Measuring forgetting \cite{jagielski2023measuring}
    - Measuring Novelty \cite{mccoy2021language}

- Here are the factors that influence memorization:
\begin{itemize}
    \item From Carlini, memorization is different than overtraining \cite{carlini2019secret}. Models can memorize arbitrary patterns (\cite{zhang2017understanding}).
    \item Capacity/size of the model \cite{carlini2023quantifying, tirumala2022memorization, jagielski2023measuring}. However, it is always memorized \cite{carlini2019secret}
    \item Data duplication \cite{carlini2023quantifying, kandpal2022deduplicating, lee2022deduplicating}
    \item Number of tokens used to prompt model \cite{carlini2023quantifying, Thomas2020InvestigatingTI}
    \item How early memorization happens \cite{carlini2019secret, biderman2023emergent, jagielski2023measuring}
    \item Nouns and verbs are memorized more \cite{tirumala2022memorization}
    \item Size of subword vocabulary (is this same as number of tokens?) \cite{kharitonov2021bpe}
    \item Model hyperparameters \cite{Thomas2020InvestigatingTI, tirumala2022memorization}
\end{itemize}

    

- Methods to reduce memorization:
\begin{itemize}
    \item Preventing overfitting (e.g. early stopping and dropout) is insufficient \cite{carlini2019secret}
    \item Data deduplication \cite{carlini2023quantifying, kandpal2022deduplicating, lee2022deduplicating}
    \item Federated learning
    \item Differential privacy \cite{carlini2019secret, ramaswamy2020training}
    \item Identifying it early \cite{biderman2023emergent}
\end{itemize}


==> writing/4mi_attacks/outline.tex <==
\subsection{Outline}

- Introduction
    - What is MI attack? Using outputs of model to infer training data membership. To be described more later, but essentially uses the confidence levels to make predictions
    - First introduced by \cite{shokri2017membership}
    - Explain practical risk of MI attack: Am I in certain voter database, genetic database, hospital info, etc.
    - Popular discourse: 
    
- Preliminaries
    - Loss based attacks
    - Label based attacks
    - Comparison to reference model
    - \cite{yu2023bag} probably has good details for this
    
- Attacks on LLMs (categorize based on type of attack?)
    - \cite{lehman2021does}: attack on BERT model w/clinical data. Fill in blank attack ("john doe's SSI is..."). "even when we constructed a variant of data in which we prepended patient names to every sentence prior to pretraining BERT, we were still unable to recover sensitive information reliably." Attacks using \cite{carlini2021extracting} are more promising but inconclusive. Code at \url{https://github.com/elehman16/exposing_patient_data_release}
    - Shadow Model
        - \cite{song2019auditing}
        - \cite{Hisamoto_2020}: attack on sequence generation model, ie output is series of text of undetermined length. Label attack, based on how many words in output match the reference. MI does not work well generally, but can in some circumstances. Similar to Song but "more realistic" as it only gets output sequence and not the probability sequence.
        - \cite{abascal2023tmi}: Transfer Membership Inference (TMI). pretraining data usually seen as non-sensitive. Using only access to fine tuned model, this attack can reveal info about pre-training set.
    - Metric
        - \cite{carlini2021extracting}: attack on GPT-2. Adversary has black box access to probability of a certain sequence and next word access. Strength of attack measured as how many examples were k-eidetic memorized and how low k was. Uses perplexity of sequence as metric. Found that MI was mostly effective on 1) trivial data such as numbers and 2) repeated substring such as "I love you". Recommends using a model comparison (see below).
        - \cite{song2020information} Embeddings transform data to low dimension that is good for ml. Among other research points, embedding models are still vulnerable to MI using similarity scores (albeit to lesser extent than non-embedded models). 30\% improvement over guessing on both word and sentence. Word embeddings: uses similarity score as metric for thresholding. Sentence embeddings: also similarity score
    - Reference Based Attack
        - \cite{mireshghallah2022quantifying}: attack on masked language models. prior studies \cite{lehman2021does, vakili2023using, jagannatha2021membership, nakamura2022kart} said MLMs are resistant to MIA. MLMs are resistant to attacks using model score but can be attacked using likelihood ratio. Adversary trains independent model from identical population. Compares log-ratio of probabilities between independent model and target model. This work adapts LRT from \cite{ye2022enhanced, murakonda2021quantifying}. \cite{goyal2022exposing} viewed MLMs as energy-based probabilistic models as used in this paper. Ratio attacks using energy increase AUC from .66 to .90 compared to baseline of metric attack using only loss
        - \cite{mattern2023membership} Reference model attacks (see mireshghalla) are effective but make unrealistic assumptions about adversary. Does an mi attack using model trained on synthetically generated "neighbor data" and shows that it still is effective.
        - \cite{carlini2021extracting} slightly different methods. 1) comparison to smaller model (important in context of memorization since they won't memorize same sequences) 2) divide by zlib compression (i.e. entropy of sequence) 3) perplexity ratio of same model trained on lowercased data (mostly same but marginally different enough) 4) 
        - \cite{Zanella_B_guelin_2020} Differential analysis (score and rank) of model before and after an update can reveal private information. Unlearning doesn't work, dp does work but at high comp cost. 


- Mitigation strategies:
    - Types of LMs:
        - \cite{jagannatha2021membership} smaller models leak less, masked LMs leak less.
        - \cite{song2020information}, embedding models leak less
    - Memorization
        - Related to MI attacks as higher memorization will lead to higher MI success. Techniques such as deduplication, federated learning, differential privacy, and early detection all help. 
        - See Memorization section. \ref{subsec:mem_mitigation}
    - Differential privacy is effective
        - Across many studies including \cite{jagannatha2021membership, abascal2023tmi, Zanella_B_guelin_2020}, DP was found to be effective
        - For more on this, see private learning section.

- Tools
    - \cite{song2019auditing} model auditing tool to help user determine if their data was used to train a model
    - \cite{marone2023data} data portraits tool. Determines if a model has already seen a training example before. 


==> writing/5private_learning/notes.tex <==


\subsubsection{Fully DP Language Models}
- \cite{anil2021largescale}
    - DP pre-training BERT
    - To ensure performance, need to massively scale up the batch sizes (2M big, $\sim 32\times$ larger than typical non-private batch size
    - Trained on Wikipedia and Books
    - MLMs typically have 70 percent accuracy. With larger batch sizes, can get up to 60 percent. Cite Figure anil batchsize.
- \cite{shi2022selective}:
    - Selective DP: policy function that determines token sensitivity. If sensitive, add noise.
    - This method showed modest improvements in model utility over standard DP-SGD while also having modest privacy improvements from canary insertion and membership inference attacks over non-private training methods.
    - \cite{zhao2022provably} showed this method isn't great especially without a perfect policy function
- \cite{zhao2022provably}
    - Extension of Shi. Done on LSTM and GPT-2.
    - Confidentially Redacted Training: alternates between dp-sgd on private and sgd on public datasets
    - On both models, reduces MIA success to near guessing levels
    - In the absence of a perfect policy function the risk of memorization is still high even with only black-box access to the model
- \cite{hoory2021dp}:
    - Develops a differentially private WordPiece tokenizer.
    - This can be used for DP pre-training as well as for applying DP to the fine-tuning, domain specific tasks. Shows strong privacy guarantees with only small dip in utility.
    - Increasing the batch size during pre-training helps with DP guarantees


\subsubsection{DP Fine-tuning of LLMs}
- \cite{kerrigan2020differentially}: First to do this
    - pre-train on public data then dpsgd fine tune is better. Only done on small feed forward networks. This is DP with respect to the fine tuning dataset only
    - Performances were compared to a GPT-2 model non-privately fine tuned. Utility was very poor due to small model size but there were improvements over doing dp for the whole thing
- \cite{li2022large}: 
    - DP on just fine-tuning portion works well
    - BERT and roBERTa models
    - Increase in batch size improves model performance. (See Figure~\ref{fig:li_hyperparameters})
    - higher learning rates and smaller clipping limits also improved model performance of a DP-SGD trained model
    - aligning the objective task with the training task improved model performance
    - \emph{ghost clipping} based on the work by \cite{lee2020scaling} eliminates memory overhead
- \cite{dupuy2022efficient}: 
    - Speeding up DP-SGD on the fine tuning portion
    - micro-batching the examples at each step. Enables GPU usage. Significant speed increases
    - CLC LSTM model \cite{ma2016end} pretrained using FastText \cite{mikolov2013fasttext} and WikiNews. also BERT on Wikipedia and One Billion Word corpus \cite{chelba2014billion}.


\subsubsection{DP predictions for LLMs}
- \cite{ginart2022submix}:
    - Considers the problem of private prediction, ie using non-private models that were fine tuned on a private corpus. Private prediction allows for application to LLMs because it doesn't require retraining the LM
    - "ensemble of LMs fine-tuned on disjoint parts of the private corpus and privatizes predictions by mixing the next-token distribution with that of a public pre-trained LM. If all models predict the same next-token distribution, then it is impossible for the next token to leak sensitive information about any unique individual so no mixing is required. By contrast, if models in the ensemble have high disagreement, SUBMIX will mix predictions with those of the public pre-trained model to minimize privacy leakage"
- \cite{majmudar2022differentially}:
    - Applied at the decoding stage. Very computationally lightweight
    - While this perturbation method is provably differentiably private, the utility tradeoff is quite significant




\subsubsection{Federated Learning}
Very few changes from first draft
- \cite{mcmahan2018learning}
- \cite{thakkar2020understanding}
- \cite{ramaswamy2020training}



Performance:
- \cite{subramani2021enabling} extensive benchmarking on dp-sgd. Does not consider LLMs but is relevant to improving performance.


==> writing/5private_learning/outline.tex <==
- Introduction

\begin{itemize}
    \item Differential Privacy \cite{dwork2006differential}. Go through main principles and ideas. \cite{dwork2018privacypreserving, dagan2020pac}. Preliminaries from \cite{majmudar2022differentially, ginart2022submix}
    \item Federated Learning: \cite{mcmahan2023communicationefficient} introduces the concept. Go through main principles and ideas. \cite{hard2019federated} FL is a promising solution towards privacy (Hard does not quantify privacy gains)
\end{itemize}

- Solution implementations (Differential privacy)
\begin{itemize}
    \item Methods for applying DP to LLMs \cite{majmudar2022differentially, ginart2022submix, mcmahan2018learning} 
    \item Go through details, results, and limitations of each
\end{itemize}

- Solutions (combined with Federated Learning)
\begin{itemize}
    \item \cite{mcmahan2018learning} uses noised federated averaging. \cite{thakkar2020understanding} and \cite{ramaswamy2020training} both also use dp federated learning
    \item Go through details, results, and limitations of each
    \item \cite{huang-etal-2020-texthide} takes a cryptographic approach. 
\end{itemize}


- Improving performance
\begin{itemize}
    \item \cite{anil2021largescale} training BERT privately reduces performance
    \item Private learning introduces additional computational costs
    \item \cite{li2022large} Ways to mitigate performance loss of private NLP
    \item \cite{dupuy2022efficient} modifications for GPU compute that improve computation time
    \item \cite{shi2022selective} masking only sensitive features improves performance on RNNs
\end{itemize}


==> writing/6copyright/outline.tex <==
\subsection{Outline}

Introduction:
- Memorization concerns lead to questions about copyright. 
    - Popular datasets often contain copyright material \cite{bandy2021addressing, biderman2022datasheet}. 
    - Preventing verbatim memorization is a false sense of security \cite{ippolito2023preventing}
- These issues are becoming more and more of an issue:
    - sarah silverman suing openai \cite{Davis2023bsilverman}
    - AI art, music, and code is booming. nobody knows what will happen with copyright \cite{Vincent2022copyright}
    - AI copyright is a major issue in WGA strike \cite{Rose2023wgacopyright}
    - WGA strike is first legal battle in oncoming labor war over ai \cite{Broderick2023wga}

Legal Discourse:
- Work by ai artists and authors are ineligible for copyright \cite{uscopyright}
- Patents by AI are ineligible for patent rights \cite{Rose2023patent}
- Fair Use doctrine governs much of the legal decisions in this space. \cite{henderson2023foundation} covers many of the details
    - 
- \cite{Sobel_2017}
- \cite{Hristov_2017}
- \cite{Sag_2019}
- \cite{Lemley_Casey_2021}
- \cite{Delacroix_2023}

Technical Solutions:
- Metrics tailored towards copyright law \cite{vyas2023provable, elkinkoren2023copyright}
- Initial methods for defining novelty or creativity \cite{franceschelli2022deepcreativity, scheffler2022formalizing}


==> writing/7unlearning/outline.tex <==
\subsection{Outline}

- Introduction
    - There are privacy risks. These are in public discourse
        - \cite{Heikkila2022gpt3} what does gpt3 know about me technology review
        - TODO: fill in...
    - Legislation is reflection this too
        - GDPR \cite{graves2020amnesiac} has good overview
        - Canada proposed CCPA
        - FTC requires deletion of models/algorithms derived from deleted data: https://www.ftc.gov/news-events/news/press-releases/2021/01/california-company-settles-ftc-allegations-it-deceived-consumers-about-use-facial-recognition-photo
    - Computational infeasibility of retraining entire models
    - Unlearning is the solution. For a more comprehensive survey on Unlearning, see \cite{nguyen2022survey}


- Preliminaries
    - Overview of unlearning from a non-technical level. Include a graphic depicting the process
    - Overview of how unlearning works with technical detail. This part covers unlearning in general given lack of in depth work on LM unlearning
    - Types of unlearning (\cite{nguyen2022survey}): exact and approximate
    - Strong vs weak unlearning algorithms \cite{neel2020descenttodelete}
    - Unlearning by efficient deletion and retraining
        - \cite{bourtoule2020machine} SISA training. 
        - \cite{graves2020amnesiac} Unlearning: replace label of sensitive data (or multiple points) with random labels. Running a few iterations of retraining is effective (TODO: is there a theoretical guarantee on this?)
    - Unlearning with gradient based methods
        - Influence functions \cite{bae2022influence}: classic technique estimating the effect of deleting a single data point. This works great for strongly convex functions such as logistic regression, but are inconsistent with neural networks.
        - Amnesiac Unlearning \cite{graves2020amnesiac}: remember which examples appeared in which training batch. During removal, undo parameter updates from those batches.
        - \cite{neel2020descenttodelete}: two sets of results: 1) gradient descent updates (+ some gaussian noise) after each add/delete request. 2) for large data dimension: bootstrap dataset, split into K parts, optimize for each and average. Gradient based updates for only deleted parts (similar to SISA)
        - \cite{jang2022knowledge}: \textit{knowledge unlearning}. Gradient ascent on chosen token sequences is sufficient
    - General reduction of unlearning problem: \cite{gupta2021adaptive}: for sequence of deletions in non-convex setting, prior work only gives guarantee for sequences chosen independent of model. If people choose to delete as a function of published model, it is adaptive. This paper gives a general reduction giving more flexible algorithms for arbitrary model classes/training methodologies



- Unlearning in LLMs
    - There is not a ton of current research on unlearning specifically within LLMs...
    - \cite{jang2022knowledge}: \textit{knowledge unlearning} as a post hoc method on pre-trained LMs. Gradient ascent on token sequences is sufficient. Sequential (rather than all at once) is better. Shows privacy guarantees
    - \cite{bourtoule2020machine}: introduces SISA training for reducing computational overhead of full model retraining. \cite{kumar2022privacy} introduces this in the NLP setting. Kumar tries unlearning on various tasks: QQP, SST, MNLI. Proposes SISA-FC and SISA-A as ways to perform guaranteed unealrning with significant reduction in time and space consumption


- Additional remarks on unlearning:
    - \cite{sekhari2021remember}: studies how many examples can be unlearned while maintaining performance. introduces algorithm that doesn't require access to training data. Quantifies limits of unlearning.
    - \cite{zhou2022fortuitous}, intentional forgetting then relearning may have benefits. Re-training after forgetting will amplify unforgotten features. ``A forgetting operation that favors the preservation of desirable features can thus be used to steer the model towards those desirable characteristics.``




